A Nonminimal Coupling Model and its Short-Range Solar System Impact

The objective of this work is to present the effects of a nonminimally coupled model of gravity on a Solar System short range regime. For this reason, this study is only valid when the cosmological contribution is considered irrelevant. The action functional of the model involves two functions $f^1(R)$ and $f^2(R)$ of the Ricci scalar curvature $R$, where the last one multiplies the matter Lagrangian. Using a Taylor expansion around $R=0$ for both functions $f^1(R)$ and $f^2(R)$, it was found that the metric around a spherical object is a perturbation of the weak-field Schwarzschild metric. The $tt$ component of the metric, a Newtonian plus a Yukawa perturbation term, is constrained using the available observational results. First it is shown that this effect is null when the characteristic mass scales of each function $f^1(R)$ and $f^2(R)$ are identical. Besides, the conclusion is that the nonminimal coupling only affects the Yukawa contribution strength and not its range and that the Starobinsky model for inflation is not experimentally constrained. Moreover, the geodetic precession effect, obtained also from the radial perturbation of the metric, reveals to be of no relevance for the constraints.

==> 0.Inicio/1.coveristfmul.tex <==
\setcounter{page}{1} \pagenumbering{Alph}

% Add PDF bookmark 
\pdfbookmark[0]{Title}{Title}

\thispagestyle{empty}
\begin{flushleft} ~\\ \vspace{-10mm} \hspace{-9mm}  \includegraphics[width=90mm, height=23mm]{Cover/istlogo} \hspace{49mm}  \includegraphics[height=23mm]{Cover/fml} 
\\ \vspace{5mm}
%~\\ \vspace{50mm} % gráficos
~\\ \begin{center} \includegraphics[height=50mm]{Cover/coverimage}  \end{center} % gráficos
~\\ \vspace{5mm}
\begin{centering}
\LARGE \textbf{Fancy Title 1}
\\ \vspace{5mm}
\Large Fancy Subtitle 1
\\ \vspace{15mm}
\Large \textbf{Full Name} \\
(Licenciado)
\\ \vspace{15mm}
\Large Dissertação para obter o grau de Mestre em
\\ \vspace{2mm}
\LARGE \textbf{Engenharia Biomédica}
\\ \vspace{20mm}

\Large \textbf{Júri}

\begin{tabular}{lcl}
\large Presidente:		&   & \large \\ 
\large Orientador: 		&   & \large \\ 
\large Co-Orientador: &   & \large \\ 
\large Vogal:	 				&   & \large \\
\end{tabular}
 
\vspace{9mm}

%\Large \textbf{\todaythesis\today} \\
\Large \textbf{Janeiro 2012} \\
\end{centering}
\let\thepage\relax
\end{flushleft}
\pagebreak


\clearpage
% Since I am using double sided pages, the second page should be white.
% Remember that when delivering the dissertation, IST requires for the cover to appear twice.

\thispagestyle{empty}
\cleardoublepage

\setcounter{page}{1} \pagenumbering{roman}

\baselineskip 18pt % line spacing: -12pt for single spacing
                   %               -18pt for 1 1/2 spacing
                   %               -24pt for double spacingnts}

==> 1.Introduction/main1.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Introduction:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Introduction}
\label{cap:int}

\section{General Relativity}
\label{sec:GR}

To study gravity, physicists rely on the theory of \ac{GR}, as they have done for almost a hundred years. \ac{GR} was developed by Einstein in 1916 and since then it has been able to demonstrate itself as a solid theory of physics. After its theoretical framework was developed, the observational confirmations didn't take long to appear: several experiments have been done to confirm it \cite{will}, such as the measure of the perihelion of Mercury, the detection of the bending of light or the E\"otv\"os torsion balances experiment, just to name a few of the classics. Besides these, also today there are people working on very recent General Relativity tests and its most dramatic consequences, such as the LAGEOS \cite{lageos} and Lunar Laser Ranging \cite{LLR} collaborations.

One of the main tenets of \ac{GR} is the relation between matter and geometry, where gravity appears not as a force field but as a deformation of the spacetime. This is mathematically represented in the \ac{EFE}, which, as all field equations in physics, are obtained from an action principle. Indeed, consider the Einstein-Hilbert action

\begin{equation}
S = \int \left[\kappa \left(R - 2\Lambda \right) + \LL_m \right] \sqrt{-g} \text{ d}^4 x,
\label{eq:einstein-hilbert_action}
\end{equation}

\noindent where $R$ is the Ricci scalar, $\LL_m$ is the matter lagrangian, $\Lambda$ stands for the Cosmological Constant, $g$ is the determinant of the metric and $\kappa$ is defined as $\kappa = c^4 / (16\pi G)$, with $G$ as Newton's constant of gravity  and $c$ as the velocity of light in a vacuum.

Hence, by the principle of least action, the variation of the action $\delta S = 0$ with respect to the metric $g^{\mu\nu}$ yields the \ac{EFE},

\begin{equation}
G_{\mu\nu} + \Lambda g_{\mu\nu} = \dfrac{1}{2\kappa} T_{\mu\nu},
\label{eq:einstein_field_equations}
\end{equation}

\noindent where $G_{\mu\nu} \equiv R_{\mu\nu} - \dfrac{1}{2} g_{\mu\nu}R $ is the Einstein tensor and $T_{\mu\nu}$ is the energy-momentum tensor of matter, clearly showing the already stated relation between matter and geometry. Applying the Bianchi identities, it is found that these equations satisfy the conservation of energy,

\begin{equation}
\nabla_\gamma G_{\mu\nu} = 0 \Rightarrow \nabla_\gamma T_{\mu\nu} = 0.
\label{eq:conversation_energy_GR}
\end{equation}

\section{Standard Cosmology and Inflation}
\label{sec:standard_cosmology}

Following the Cosmological Principle, which states that the universe is homogeneous and isotropic, the universe can be said to have a \ac{FLRW} metric \cite{walker,robertson}:

\begin{equation}
ds^2 = - dt^2 + a^2(t) \left( \dfrac{dr^2}{1 - K r^2} + r^2 d\Omega^2 \right)
\label{eq:metric_flrw},
\end{equation}

\noindent where $a(t)$ is the cosmological scale factor, $d\Omega^2$ is the line element for the 2-sphere and $K$ is related to the curvature of the spatial section of spacetime, where the spatial coordinates are comoving coordinates.

One may consider that at very large scales the universe can be described as being a perfect fluid, endowed with an energy-momentum tensor

\begin{equation}
T_{\mu\nu} = \left(\rho + p \right) u_\mu u_\nu - p g_{\mu\nu},
\label{eq:tensor_perfect_fluid}
\end{equation}

\noindent where $\rho$ is the energy density, $p$ is the pressure and $u_\mu$ is the 4-velocity vector. Inserting this tensor and the metric \eqref{eq:metric_flrw} into the \ac{EFE} \eqref{eq:einstein_field_equations} gives the cosmology structure equations:

\begin{eqnarray}
\dot{a}^2 + K c^2 &=& \dfrac{a^2}{3} \left( 8 \pi G \rho + \Lambda c^2 \right), \label{eq:friedmann_eq_1}\\
\dfrac{\ddot{a}}{a} &=& - \dfrac{4 \pi G}{3}\left( \rho + \dfrac{3 p}{c^2}\right) + \dfrac{\Lambda c^2}{3},
\label{eq:cosmology_structure_equations}
\end{eqnarray}

\noindent where $\dot{a}=da/dt$. The first of these equations is called the Friedmann equation. Through a simple manipulation, both these equations can be written in the form of the conservation of energy:

\begin{equation}
\dot{\rho} + 3 H \left( \rho c^2 + p \right) \Leftrightarrow
\dfrac{d}{dt} \left( \rho c^2 a^3 \right) + p \dfrac{d}{dt} a^3 = 0,
\label{eq:conservation_energy_cosmology}
\end{equation}

\noindent which can also be directly obtained from Eq. \eqref{eq:conversation_energy_GR}. The Hubble parameter is extremely useful to characterize the evolution of the universe and is defined as

\begin{equation}
H = \dot{a} / a.
\label{eq:hubble_parameter}
\end{equation} 

The above equations \eqref{eq:friedmann_eq_1} and \eqref{eq:cosmology_structure_equations} yield a full description of the structure and development of the universe if an \ac{EOS} is known. The simplest approach is to consider a barotrope, described by the equation

\begin{equation}
p = w \rho,
\label{eq:eos_standard}
\end{equation}

\noindent where $w$ is a constant independent of time. Notice that inserting this \ac{EOS} into the conservation of energy \eqref{eq:conservation_energy_cosmology} yields

\begin{equation}
\dfrac{\dot{\rho}}{\rho} = - 3 \left( 1 + w \right) H.
\end{equation}

\noindent This expression can be integrated to obtain the solution of $\rho$,

\begin{equation}
\rho (a) = \rho_0 a^{-3 \left(1 + w \right)},
\end{equation}

\noindent where $\rho_0$ is the value of the energy density at the present time $t_0$, when $a(t_0) \equiv a_0$.

The universe underwent different stages of evolution, characterized by the dominance of different kinds of matter, in the so-called radiation, matter and dark energy eras. In the radiation era the Universe was dominated by electromagnetic radiation or massive particles travelling at velocities close to the speed of light, so that its \ac{EOS} is

\begin{equation}
p_r = \dfrac{1}{3} \rho_r.
\end{equation}

\noindent The energy density in the radiation era falls off as $\rho_r \propto a^{-4}$. As for the matter era, dominated by nonrelativistic particles with approximately no collisions, matter has essentially zero pressure $p_m =0$, so that $w_m=0$. In this case the energy density falls off as $\rho_m \propto a^{-3}$.

Knowing how the energy density behaves with the scale factor, it is possible to derive the function $a(t)$ through the Friedmann equation \eqref{eq:friedmann_eq_1} and the Hubble parameter definition \eqref{eq:hubble_parameter}. Considering a flat model $K=0$ with $\Lambda = 0$, in the radiation era the scale factor becomes $a(t) \propto t^{1/2}$ and in the matter era, $a(t) \propto t^{2/3}$. It should also be mentioned that when a non-vanishing cosmological constant $\Lambda \neq 0$ dominates, so that $\rho_\Lambda = -p_\Lambda$ (i.e. $\omega_\Lambda =-1$), one obtains
$\rho_\Lambda \propto a$, so that $a(t) \propto \exp (Ht)$. When the universe behaves according to the latter model it means that it is going through a De Sitter phase, which characterizes the dark energy era.

The standard Big-Bang model, described by Eqs. \eqref{eq:cosmology_structure_equations} and \eqref{eq:friedmann_eq_1}, has seen many of its predictions confirmed by cosmological observations, such as the galaxies red-shift or the detection of the \ac{CMB} \cite{weinberg}. Nonetheless, some observations showed that there were three problems in this model. They were the horizon problem, related to the explanation of how regions of the universe not causally related were in thermal equilibrium, as shown by the \ac{CMB} Radiation, the flatness problem, from the extreme fine-tuning necessary to explain how the universe is as spatially flat as it looks, and the monopole problem, indicating that these exotic entities should dominate the universe in the present time, contrary to observations. These three problems were solved in a single theory, called inflation \cite{guth}.

The theory of inflation comes directly from the solution to the flatness problem. Defining the critical density as 

\begin{equation}
\rho_c(t) = 3 H^2 \slash 8 \pi G,
\label{eq:critical_density}
\end{equation}

\noindent and neglecting the cosmological constant term, the Friedmann equation \eqref{eq:friedmann_eq_1} can be written as

\begin{equation}
\left| \Omega - 1 \right| = \dfrac{|K|c^2}{a^2 H^2} = \dfrac{\left| K \right| c^2}{\dot{a}^2} ,
\label{eq:friedmann_eq_2}
\end{equation}

\noindent where $\Omega$ is the density parameter defined as $\Omega = \rho \slash \rho_c$. The standard cosmological model predicts that the $r.h.s.$ of the above equation should increase with time, hence $\Omega$ should become larger with time since the Big Bang, but observations yield an $\Omega \sim 1$, i.e. the universe is flat ($K=0$). The only way to counter this would be for the $r.h.s.$ to decrease with time:

\begin{equation}
\dfrac{\left| K \right| c^2}{\dot{a}^2} \text{ should decrease } \Rightarrow \dot{a} \text{ should increase } \Rightarrow \ddot{a} > 0,
\label{eq:inflation_condition}
\end{equation}

\noindent which is the inflation condition.

The origin of inflation is explained by means of a scalar field named inflaton, $\phi$, whose effective energy density and pressure are written as

\begin{equation}
\rho_\phi = \dfrac{\dot{\phi}^2}{2} + V(\phi), \qquad\qquad\qquad
p_\phi = \dfrac{\dot{\phi}^2}{2} - V(\phi),
\label{eq:energy_pressure_phi}
\end{equation}

\noindent where the potential $V(\phi)$ depends on the inflation model in question. Moreover, the inflation condition means that the potential energy must dominate in order to obtain a phase of accelerated expansion,

\begin{equation}
\ddot{a} > 0 \Leftrightarrow p < -\rho c^2 \slash 3 \Leftrightarrow \dot{\phi}^2 < V(\phi),
\label{eq:potential_dominates_inflation}
\end{equation}

\noindent where the second cosmology structure equation \eqref{eq:cosmology_structure_equations} was used.
This is the so-called \ac{SRA}, which states that the kinetic term can be neglected with respect to the potential term. Notice that if this condition applies, then by Eq. \eqref{eq:energy_pressure_phi}, the \ac{EOS} becomes similar to that of a Cosmological Constant, $\rho_\phi \simeq -p_\phi$. Inserting the inflaton energy density and pressure \eqref{eq:energy_pressure_phi} into the Friedmann equation \eqref{eq:friedmann_eq_1} and the energy conservation \eqref{eq:conservation_energy_cosmology} gives the inflation structure equations:

\begin{eqnarray}
H^2 &=& \dfrac{8\pi G}{3} \left[ V(\phi) + \dfrac{\dot{\phi}^2}{2}\right], \\
\ddot{\phi} +3 H \dot{\phi} &=& - V'(\phi), \label{eq:conservation_eq_inflation}
\end{eqnarray}

\noindent where $V'(\phi) = dV \slash d\phi$. By the \ac{SRA}, these equations become

\begin{eqnarray}
H^2 &\simeq & \dfrac{8 \pi G}{3} V(\phi), \\
3 H \dot{\phi} &\simeq & - V'(\phi).
\end{eqnarray}

\noindent It is also possible to define the slow-roll parameters as

\begin{eqnarray}
\epsilon (\phi) &=& \dfrac{1}{16 \pi G} \left( \dfrac{V'}{V} \right)^2 \ll 1, \\
\left|\eta (\phi) \right| &=& \left| \dfrac{1}{8\pi G} \dfrac{V''}{V} \right| \ll 1,
\end{eqnarray}

\noindent which measure the slope and the curvature of $V(\phi)$, respectively. Their smallness is necessary to satisfy the \ac{SRA}.

The number of $e$-folds between an initial $\phi_i$ and final state $\phi_f$ of the inflation is determined by

\begin{equation}
N = \ln \dfrac{a(t_f)}{a(t_i)} = \int^{t_f}_{t_i} H dt = -8 \pi G \int^{\phi_f}_{\phi_i} \dfrac{V}{V'} d\phi,
\end{equation}

\noindent where $dt=d\phi/\dot{\phi}$ was used. It is known that for inflation to overcome the three original problems of the standard cosmological model, $N$ should be no less than $70$ \cite{felice}.

The duration of inflation is the time when the \ac{SRA} is valid, a period in which the energy density and temperature of the universe are extremely low. As such, at the end of inflation, the potential $V(\phi)$ loses its strength and the universe must go through a reheating process, as the exponential expansion has left the Universe at essentially zero temperature. This is achieved through an oscillation of the inflaton in a potential well, as shown in figure \ref{fig:inflation_potential}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth]{fig1.pdf}
\caption{Typical inflation potential. Adapted from Ref. \cite{reheatingpic}.}
\label{fig:inflation_potential}
\end{figure}

Quantum field theory explains that an oscillating electric field produces electron-positron pairs; similarly, the oscillation of the field $\phi$ produces its own particles, with the energy that it is losing until the end of the oscillations. This will happen until the temperature needed to go back to the standard cosmological model is reached. Such a process is explained in a more analytical way through the conservation of energy inflation equation \eqref{eq:conservation_eq_inflation}, by adding the term $\Gamma_\phi$, which is the decay range of $\phi$:

\begin{equation}
\ddot{\phi} + 3H\dot{\phi} + \Gamma_\phi \dot{\phi} + V'(\phi) = 0.
\label{eq:oscillation_reheating}
\end{equation}

\noindent This can be interpreted as a friction term, where the energy lost by the inflaton is transferred to the particles produced, thus reheating the Universe.

Without entering into much details, inflation has already some observational evidences, such as the last year results from the Planck experiment \cite{planckinflation} and the very recent clues of evidence of gravitational waves \cite{bicep2}.


\section{Modern Problems}
\label{sec:mod_problems}

Besides the exact origins of inflation, other problems still remain to be explained, such as the relation between quantum mechanics and gravity (check Ref. \cite{quantumgravity} for a review on the subject) and the nature of dark matter and dark energy. These concepts arise as an explanation to an observational effect that is contrary to the theoretical prevision of \ac{GR}. Dark Matter is inferred, for example, from the anomalous flattening of the galaxy rotation curves: at the periphery of galaxies, the rotation velocity of each galaxy should be much slower than observed, hence there should be some dark ($i.e.$ unseen, electromagnetically invisible) matter that yields this gravitational effect. There are other observational evidences that show this effect, which can be found in Ref. \cite{darkmatter1}, where some of the candidates to dark matter and detection methods are also explained. 

Dark energy, on the other hand, is related to the cosmological scale of the universe. In the late 1990s, the observation of the red-shift of distant supernovae became the main evidence for the accelerated expansion of the universe \cite{perlmutter,riess}. Unexplained by visible matter in the standard cosmological model, many solutions have been proposed, commonly known as dark energy. Indeed, as the moving force of the accelerated expansion, recent observations have concluded dark energy to be $68,3\%$ of all the matter in the universe, with dark matter being $26,8\%$ and baryonic ($i.e.$ ordinary) matter $4,9\%$ \cite{planck}.

Another explanation for the accelerated expansion are alternative theories of gravity, showing that the accelerated expansion might be the door for a generalization of Einstein's theory of gravity. Amongst these proposals, the focus in this work will be the so-called $f(R)$ theories, which will be introduced in the following chapter, and also include nonminimal coupling theories, also developed here.


\cleardoublepage

==> 100.Bibliography/bibliography.tex <==
\begin{thebibliography}{9}

\bibitem{nunocb} N. Castel-Branco, J. P\'aramos and R. March,
		Perturbation of the metric around a spherical body from a nonminimal coupling between matter and curvature,
		Submitted to Physics Letters B, arXiv:1403.7251

\bibitem{will} C. M. Will,
		The Confrontation between general relativity and experiment,
		Living Rev. Rel. 9 (2006) 3.
		GR-QC/0510072    
		
\bibitem{lageos} D. M. Lucchesi and R. Peron,
		Accurate Measurement in the Field of the Earth of the General-Relativistic Precession of the LAGEOS II Pericenter and New Constraints on Non-Newtonian Gravity,
		Phys. Rev. Lett. 105 (2010), 231103                  
		
\bibitem{LLR} J. Mueller, J. G. Williams, S. G. Turyshev,
		Lunar Laser Ranging Contributions to Relativity and Geodesy,
		"Lasers, Clocks, and Drag-Free: Technologies for Future Exploration in Space and Tests of Gravity", H. Dittus, C. Laemmerzahl, S. Turyshev, eds. pp. 357-372 (Springer Verlag, 2006)

\bibitem{walker} A. G. Walker,
		On Riemannian Spaces with Spherical Symmetry about a Line and the Conditions of Isotropy in General Relativity,
		Q. J. Math (1935) os-6 (1): 81-93.
		\href{http://qjmath.oxfordjournals.org/content/os-6/1/81.full.pdf}{doi:10.1093/qmath/os-6.1.81}
		
\bibitem{robertson} H. P. Robertson,
		Kinematics and World-Structure,
		Astrophys.J. 82 (1935) 284.
		\href{http://dx.doi.org/10.1086/143681}{doi:10.1086/143681}
				
\bibitem{reheatingpic} Baumann et al.,
		CMBPol Mission Concept Study - Probing Inflation with CMB Polarization	,
		AIP Conference Proceedings, 1141, 10-120 (2009),
		DOI:http://dx.doi.org/10.1063/1.3160885

		
\bibitem{planckinflation} P.A.R. Ade and others,
		Planck 2013 results. XXII. Constraints on inflation,
		Planck Collaboration (2013), arXiv 1303.5082.
		
\bibitem{bicep2} P.A.R. Ade and others,
		BICEP2 I: Detection Of B-mode Polarization at Degree Angular Scales,
		BICEP2 Collaboration (2014), arXiv 1403.3985.
		
\bibitem{darkmatter1} G. Bertone, D. Hooper, and J. Silk,
		Particle dark matter: evidence, candidates and constraints,
		Physics Reports 405 (Jan, 2005) 279.
		\href{http://arxiv.org/abs/hep-ph/0404175}{arXiv:hep-ph/0404175}
		\href{http://www.sciencedirect.com/science/article/		 pii/S0370157304003515}{10.1016/j.physrep.2004.08.031}
	
\bibitem{quantumgravity} C. Kiefer, 
		\emph{Quantum Gravity}, Third Edition,
		Oxford University Press, 2012
	
\bibitem{perlmutter} S. Perlmutter, et al.,
		Measurements of Omega and Lambda from 42 high redshift supernovae,
		Astrophys.J. 517 (1999) 565.
		\href{http://iopscience.iop.org/0004-637X/517/2/565/}{doi:10.1086/307221}
		\href{http://arxiv.org/abs/astro-ph/9812133}{arXiv:astro-ph/9812133}
		
\bibitem{riess} A. G. Riess, et al.,
		Observational evidence from supernovae for an accelerating universe and a cosmological constant,
		Astron.J. 116 (1998) 1009.
		\href{http://iopscience.iop.org/1538-3881/116/3/1009/}{doi:10.1086/300499}
		\href{http://arxiv.org/abs/astro-ph/9805201}{arXiv:astro-ph/9805201}

\bibitem{planck} P. A. R. Ade, et al,
		Planck 2013 results. I. Overview of products and scientific results,
		\href{http://arxiv.org/abs/1303.5062}{arXiv:1303.5062}.
		
\bibitem{darkenergyreview} E. J. Copeland, M. Sami and S. Tsujikawa,
		Dynamics of dark energy,
		Int.J.Mod.Phys. D15 (2006) 1753-1936.
		
\bibitem{capozziello1} S. Capozziello, V. Cardone and A. Troisi,
		Reconciling dark energy models with $f(R)$ theories,
		Phys. Rev. D 71, 043503 (2005).
		
\bibitem{lovelock} D. Lovelock,
		The Einstein Tensor and Its Generalizations,
		J. Math. Phys. 12, 498 (1971)
		
\bibitem{koivisto} T. Koivisto,
		Covariant conservation of energy-momentum in modified gravities,
		Class. Quant. Grav. 23, 4289 (2006).
		
\bibitem{bransdicke} C. Brans and R. H. Dicke,
		Mach's Principle and a Relativistic Theory of Gravitation,
		Phys. Rev. 124 (1961) 925-935.
		\href{http://journals.aps.org/pr/abstract/10.1103/PhysRev.124.925}{10.1103/PhysRev.124.925}
		
\bibitem{capozziello2} S. Capozziello, R. de Ritis and A. A. Marino,
		Some aspects of the cosmological conformal equivalence between ``Jordan Frame'' and ``Einstein Frame'',
		Class. Quant. Grav. 14:3243-3258 (1997).
		
\bibitem{faraoni1} V. Faraoni, E. Gunzig and P. Nardone,
		Conformal transformations in classical gravitational theories and in cosmology,
		Fund. Cosmic Phys. 20:121 (1999).
		
\bibitem{guth} A. H. Guth,
		The Inflationary Universe: A Possible Solution to the Horizon and Flatness Problems,
		Phys. Rev D \textbf{23} 2 (1981) 347.
		\href{http://journals.aps.org/prd/pdf/10.1103/PhysRevD.23.347}{10.1103/PhysRevD.23.347}		
		
\bibitem{liddle} A. Liddle,
		\emph{An Introduction to Modern Cosmology},
		England: John Wiley \& Sons Ltd, 2nd edition (2003).

\bibitem{linde} A. Linde,
		Inflationary Cosmology,
		Lect. Notes Phys. 738:1-54 (2008)

\bibitem{felice} A. D. Felice and S. Tsujikawa,
		$f(R)$ Theories,
		Living Rev. Rel. 13 (2010) 3.
		\href{http://www.livingreviews.org/lrr-2010-3}{lrr-2010-3}

\bibitem{starobinsky} A. A. Starobinsky,
		A new type of isotropic cosmological models without singularity,
		Phys. Lett. B 91 (1980) 99-102.
		\href{http://dx.doi.org/10.1016/0370-2693(80)90670-X}{doi.10.1016/0370-2693(80)}
		
\bibitem{wmap} E. Komatsu et al. (WMAP Collaboration),
		``Five-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation",
		Astrophys. J. Suppl. Ser., 180, 330-376 (2009).
		
\bibitem{dynimpac1} O. Bertolami, F. S. N. Lobo and J. P\'aramos,
		Nonminimal coupling of perfect fluids to curvature
		Phys. Rev. D \textbf{78}, 064036 (2008).
		
\bibitem{adelberg2} D. J. Kapner, T. S. Cook, E. G. Adelberger, J. H. Gundlach, B. R. Heckel, C. D. Hoyle, and H. E. Swanson,
		Particle-Physics Implications of a Recent Test of the Gravitational Inverse-Square Law,
		 Phys. Rev. Lett. 98, 021101 (2007)

\bibitem{reheating_detail} M. B. Mijic, M. S. Morris and W. M. Suen,
		The $R^2$ cosmology: Inflation without a phase transition,
		Phys. Rev. D 34 (1986) 2934.
		
\bibitem{mathieu_map1} L. Kofman, A. Linde, and A. A. Starobinsky,
		Reheating after Inflation,
		Phys. Rev. Lett. 73 (1994) 3195.
				
\bibitem{reheating} O. Bertolami, P. Fraz\~ao, J. P\'aramos,
				\emph{Reheating via a generalized nonminimal coupling of curvature to matter},
				\emph{Phys. Rev.} \textbf{D 83}, 044010 (2011)
				
\bibitem{chiba} T. Chiba, T. L. Smith, A. L. Erickcek,
				Solar System constraints to general $f(R)$ gravity,
				\emph{Phys. Rev.} \textbf{D 75} 124014 (2007)
				
\bibitem{naff} J. N\"aff, P. Jetzer,
				\emph{On the $1/c$ expansion of $f(R)$ gravity},
				\emph{Phys. Rev.} \textbf{D 81}, 104003 (2010)
		
\bibitem{solar} O. Bertolami, R. March and J. P\'aramos,
		Solar System Constraints to Nonminimally Coupled Gravity
		Phys. Rev. D 88, 064019 (2013).
		
\bibitem{ChibaReview} T. Chiba,
		The Constancy of the Constants of Nature: Updates,
		Prog. Theor. Phys. {\bf 126}, 993 (2011).
		
\bibitem{nmcexpand} O. Bertolami, P. Fraz\~ ao and J. P\'aramos,
		Accelerated expansion from a non-minimal gravitational coupling to matter,
		Phys. Rev. D 81, 104046 (2010).
		
\bibitem{capozziello3} S. Capozziello, V F. Cardone, S. Carloni, A. Troisi,
		Curvature quintessence matched with observational data,
		Int. J. Mod. Phys. D12 1969-1982 (2003).
		
\bibitem{cassini} B. Bertolli, L. Iess and P. Tortora,
		A test of general relativity using radio links with the Cassini spacecraft,
		Nature 425, 374-376 (2003).

\bibitem{statusgr} O. Bertolami and J. P\'aramos,
		``The experimental status of Special and General Relativity'',
		to appear in {\it Handbook of Spacetime}, Springer, Berlin (2013);			arXiv:1212.2177 [gr-qc].

\bibitem{fischbach} E. Fischbach and C. L. Talmadge,
		``{\it The Search for Non-Newtonian Gravity},
		Springer Verlag, 1999.
		
\bibitem{adelberg1} E. G. Adelberger, B. R. Heckel and A. E. Nelson,
		Tests Of The Gravitational Inverse-Square Law,
		Annu. Rev. Nucl. Part. Sci. {\bf 53}, 77 (2003).
		
\bibitem{salumbides} E. J. Salumbides, W. Ubachs and V. I. Korobov,
		Bounds on fifth forces at the sub-\AA\ length scale
		arXiv:1308.1711 [hep-ph].
		
\bibitem{adelberg3} E.G. Adelberger, J.H. Gundlach, B.R. Heckel, S. Hoedl, S. Schlamminger,
		Torsion balance experiments: A low-energy frontier of particle physics,
		Prog. Part. Nucl. Phys. 62, 102 (2009).
		
\bibitem{talmadge} C. Talmadge, J.-P. Berthias, R. W. Hellings, and E. M. Standish,
	Model-Independent Constraints on Possible Modifications of Newtonian Gravity,
	Phys. Rev. Lett. 61, 1159 (1988).
	
\bibitem{nordtvedt} K. Nordtvedt,
		Equivalence principle for massive bodies. II. Theory, 
		Phys. Rev., 169, 1017-1025, (1968).
	
\bibitem{willbook} C. M. Will,
		Theory and experiment in gravitational physics,
		(Cambridge University Press, Cambridge, U.K.; New York, U.S.A., 1993), 2nd edition.
		
\bibitem{feynman} R. P. Feynman, R. B. Leighton, M. Sands,
		\emph{The Feynman Lectures on Physics},
		Basic Books, The New Millenium Edition edition (2010)
		
\bibitem{weinberg} S. Weinberg,
		\emph{Gravitation and Cosmology: Principles and Applications of the General Theory of Relativity},
		Springer-Verlag, Berlin (1972)

\bibitem{GPB} C.W.F.Everitt, D.B.DeBra, B.W.Parkinson, J.P.Turneaure, J.W.Conklin, M.I.Heifetz, G.M.
Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak, M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. G. Solomonik, K. Stahl, P. W. Worden, W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa, J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,
		Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,
		Phys. Rev. Lett. 106 (2011) 221101.

\bibitem{gpbwill} C. M. Will,
		Finally, results from Gravity Probe B,
		Physics 4, 43 (2011).
		
\bibitem{gpbteam} Gravity Probe B Team, Stanford, NASA,
		http://einstein.stanford.edu/highlights/status1.html	
		
\bibitem{stelobserv} O. Bertolami, J. P\'aramos,
				\emph{Do $f(R)$ theories matter?}, 
				\emph{Phys. Rev.} \textbf{D 77}, 084018 (2008)
				
\bibitem{gravcollapse} J. P\'aramos, C. Bastos,
		Gravitational collapse in non-minimally coupled gravity: finite density singularities and the breaking of the no-hair theorem,
		Phys. Rev. D86 (2012) 103007.
		
\bibitem{NASAprofile} {\it http://spacemath.gsfc.nasa.gov}

\bibitem{matching} T. Clifton, P. Dunsby, R. Goswami, A. M. Nzioki,
		On the absence of the usual weak-field limit, and the impossibility of embedding some known solutions for isolated masses in cosmologies with f(R) dark energy,
		Phys.Rev. D87 (6) (2013) 063517.
		
\bibitem{darkmatter} M. Sereno, P. Jetzer,
		Dark matter versus modifications of the gravitational inverse-square law: results from planetary motion in the solar system,
		Monthly Notices of the Royal Astronomical Society 371 (2) (2006), 626-632.
		
\bibitem{Clifton} T. Clifton,
		Parametrized post-newtonian limit of fourth-order theories of gravity,
		Phys. Rev. D 77 (2008) 024041.
		
\bibitem{analogy1}P. Teyssandier and P. Tourranc,
		The 	Cauchy problem for the $R+R^2$ theories of gravity without torsion,
		J. Math. Phys. {\bf 24} 2793 (1983); 

\bibitem{analogy2} H. Schmidt,
		Variational derivatives of arbitrarily high order and multiinflation cosmological models,
		Class. Quant. Grav. {\bf 7} 1023 (1990);
	
\bibitem{analogy3} D. Wands,
		Extended gravity theories and the Einstein-Hilbert action,
		Class. Quant. Grav. {\bf 11} 269 (1994).
		
\bibitem{mimlambda} O. Bertolami and J. P\'aramos,
		Mimicking the cosmological constant: Constant curvature spherical solutions in a non-minimally coupled model,
		Phys. Rev. D \textbf{84}, 064022 (2011).

\bibitem{dynimpac2} O. Bertolami and J. P\'aramos,
		Homogeneous spherically symmetric bodies with a nonminimal coupling between curvature and matter: the choice of the Lagrangian density for matter,
		arXiv:1306.1177 [gr-qc].
		
\bibitem{chameleon1} J. Khoury and A. Weltman,
		Chameleon cosmology,
		Phys. Rev. {\bf D69}, 044026 (2004).
		
\bibitem{chameleon2} J. Khoury and A. Weltman,
		Chameleon fields: Awaiting surpreses for tests of gravity in space,
		Phys. Rev. Lett. {\bf 93}, 171104 (2004).
		
\bibitem{chameleon3} T. Waterhouse,
		An Introduction to Chameleon Gravity,
		astro-ph/0611816.

\bibitem{chameleon4} P. Brax, C. Vandebruck and A. Davis,
		A Chameleon Primer,
		astro-ph/0706.1024.

\bibitem{multiscalar} O. Bertolami and J. P\'aramos,
		On the non-trivial gravitational coupling to matter,
		Class. Quant. Grav. \textbf{25}, 245017 (2008).



				

\end{thebibliography}


==> 2.Chapter/1.sectiona.tex <==
\section{Section A}
\label{sec:sectiona}

\subsection{Subsection A}
\label{subsec:subasectionA}

This would be a citation \cite{dummy}.

\ac{acro} 
% The first time you use this, the acronym will be written in full with the acronym in parentheses: supernova (SN). At later times it will just print the acronym: SN.

\acf{acro}
% written out form with acronym in parentheses, irrespective of previous use

\acs{acro}
% acronym form, irrespective of previous use

\acl{acro}
% written out form without following acronym

\acp{acro}
% plural form of acronym by adding an s. \acfp. \acsp, \aclp work as well.

As seen in \cite{wiki}. \emph{Enfatizar}

\subsection{Subsection B}
\label{subsec:subbsectiona}

\begin{figure}[H]
	\centering
		\includegraphics[width=0.5\linewidth]{2.Chapter/dummy.pdf}
	\caption[Dummy Figure Caption for List of Figures.]{Dummy Figure Caption.}
	\label{fig:dummyfigure1}
\end{figure}

Remember you can change the reference style. Another dummy citation \cite{site}.

==> 2.Chapter/2.sectionb.tex <==
\section{Section B}
\label{sec:sectionb}

\subsection{Subsection A}
\label{subsec:subasectionB}

The model described can also be represented as

\begin{equation}
\dot{\mathbf{x}}(t) = \mathbf{T}\mathbf{z}(y),\  \mathbf{y}(0) = \mathbf{y}_0,\  z\geq 0 \\
\label{eq:dummyeq1}
\end{equation}

\noindent where

\begin{equation}
\mathbf{A} = \left[ \begin{array}{cc} -(a_{12} + a_{10}) & a_{21} \\ a_{12} & -(a_{21} + a_{20}) \end{array} \right],\ \mathbf{x} = \left[ \begin{array}{c} x_1 \\ x_2 \end{array} \right] \\
\label{eq:dummyeq2}
\end{equation}


\subsection{Subsection B}
\label{subsec:subbsectionB}

\begin{table}[H]
	\centering
	\caption{Dummy Table.}
	\begin{tabular}{|c|c|c|c|} \hline
		\textbf{Vendor Name} 				& \textbf{Short Name}	& \textbf{Commercial Name}	& \textbf{Manufacturer}	\\ \hline \hline
		\multirow{3}{*}{Text in Multiple Row}		&	ABC				&  ABC\textreg				& ABC SA			         \\ \cline{2-4}
		 								&        DEF				&  DEF\textreg				& DEF SA				\\ \cline{2-4}
										&        GHF			&  GHF\textreg				& GHF SA				\\ \hline
		Text in Single Row					&        IJK				& IJK\textreg				& IJK SA				\\ \hline
		Frescos SA						&        LMN			& LMN\textreg				& LMN SA				\\ \hline
		Carros Lda.						&    \multicolumn{3}{|c|}{Text in Multiple Column}							\\ \hline
	\end{tabular}
	\label{tab:dummytable}
\end{table}

==> 3.Chapter/main,_old.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dummy Chapter:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% f(R) theories:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Nonminimal Coupling}
\label{cap:nmc}

The remarkable range of applications of $f(R)$ gravity, and in particular the Starobinsky inflationary model, prompted physicists to generalize these theories even further. This generalization is made by a \ac{NMC} between geometry and matter, through the product of the matter Lagrangian density with another function of the curvature, as posited by the action

\begin{equation}\label{eq:action_nmc}
S_\text{NMC}=\int \left[\dfrac{1}{2} f^1(R)+\left[1+f^2(R)\right] \LL_m\right]
\sqrt{-g} d^4x.
\end{equation}

\noindent The field equations, obtained through the variation of the action with respect to the metric, are

\begin{equation} \label{eq:field_equations_nmc}
\left(f^1_R + 2 f^2_R \LL_m \right) R_{\mu \nu} -
\dfrac{1}{2} f^1 g_{\mu \nu} =
\left(1+ f^2 \right) T_{\mu \nu} +\left( \square_{\mu \nu} - g_{\mu \nu} \square \right)
\left( f^1_R + 2 f^2_R \LL_m \right),
\end{equation}

\noindent where $G_{\mu\nu}$ is the Einstein tensor, $f_R^i \equiv df^i /dR$ and $\triangle_{\mu\nu} \equiv \nabla_\mu \nabla_\nu - g_{\mu\nu} \square$. If $f^1(R) = 2 \kappa ( R - 2\Lambda)$ and $f^2(R) = 0$, then the action \eqref{eq:action_nmc} collapses to the Einstein-Hilbert action from \eqref{eq:einstein-hilbert_action}.

It should be said that, in opposition to \ac{GR} and pure $f(R)$ gravity, these field equations do not respect the conservation of energy law, $\nabla^\mu T_{\mu\nu} \neq 0$. Indeed, the covariant derivative of the field equations \eqref{eq:field_equations_nmc}, together with the Bianchi identities $\nabla^\mu G_{\mu\nu} = 0$ and the identity

\begin{equation}
(\square \nabla_\nu - \nabla_\nu \square ) f_R^i = R_{\mu\nu} \nabla^\mu f_R^i,
\end{equation}

\noindent yields for the covariant derivative of the energy-momentum tensor,

\begin{equation}
\nabla^\mu T_{\mu\nu} = \dfrac{f_R^2}{1+f^2} \left(g_{\mu\nu} \LL_m - T_{\mu\nu} \right) \nabla^\mu R.
\end{equation}

\noindent Nonetheless, if $f^2(R) = 0$, the pure $f(R)$ case is recovered and the conservation law is fulfilled. This non-conservation of the energy-momentum tensor may yield a violation of the Equivalence principle, for the nonminimal coupling between geometry and matter means that the motion of matter is dependent on the specific form of the Lagrangian density $\LL_m$ and thus matter may not follow the expected geodesic motion.

\section{Scalar-fields equivalence}
\label{sec:scalar-fields}

In section \ref{sec: scalar-fields equiv}, the pure $f(R)$ gravity theories were shown to be equivalent to scalar-tensor theories $-$ in particular, to a \ac{BD} theory of gravity. \ac{NMC} theories of gravity can also be written in a similar way, though with two independent scalar fields. These theories are introduced through the action

\begin{equation}
S = \int \left[ \dfrac{1}{2} f^1 (\phi) + \left[ 1 + f^2 (\phi) \right] \LL_m + \psi (R - \phi) \right] \sqrt{-g} d^4 x,
\label{eq:action_scalar_field_nmc}
\end{equation}

\noindent where $\psi$ acts as a Lagrange multiplier imposing the relation $\phi = R$, with which the action $S$ is reduced to $S_{NMC}$. The variation of this action \eqref{eq:action_scalar_field_nmc} with respect to $\phi$ then yields

\begin{equation}
\psi = \dfrac{1}{2} f^1_R (\phi) + f_R^2 (\phi) \LL_m,
\end{equation}

\noindent which indicates that both scalar-fields are independent if $\LL_m \neq 0$ or $f_R^2 \neq 0$. If $f_R^2=0$, then the action returns to the pure $f(R)$ case.

As in the pure $f(R)$ situation, the action \eqref{eq:action_scalar_field_nmc} can be written in the form of a \ac{BD} theory with $\omega_{BD} = 0$ (check Eq. \eqref{eq:action_brans_dicke}) and the same scalar-fields,

\begin{equation}
S = \int \left[ \psi R - V(\phi,\psi) + \left[ 1 + f^2(\phi) \right] \LL_m \right] \sqrt{-g} d^4x,
\end{equation}

\noindent with the potential

\begin{equation}
V(\phi,\psi) = \phi \psi - \dfrac{1}{2} f^1 (\phi).
\end{equation}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Preheating and Inflation}
\label{sec:preheating}

In section \ref{sec:reheating}, the process of particle production after inflation was explained by means of a preheating mechanism, whose main characteristic was on the parametric resonance of a quantum field $\chi$. The action of this field included a \ac{NMC} term between the curvature and the field itself, of the type $\xi R \chi^2$ $-$ \textit{i.e.} an additional mass term. This linear \ac{NMC} prompts for the more general assumption of the action \eqref{eq:action_nmc} with the functions

\begin{equation}
f^1(R) = 2\kappa \left( R + \dfrac{R^2}{6 M^2} \right), ~~~\qquad\qquad~~~~~~ f^2(R) = 2\xi \dfrac{R}{M^2}.
\end{equation}

\noindent Logically, this specific action has to be able to explain inflation at the standard \ac{SRA}, which means that $f^2(R)$ should interfere only in the preheating situation, and so the \ac{NMC} model only works as part of a perturbative regime with $f^2(R) \sim 0$.

As stated in section \ref{sec:starobinsky}, the mass parameter has the value $M \sim 10^{13}$ GeV$/c^2$, whereas the \ac{NMC} parameter $\xi$ is dimensionless and subject to the range $1 < \xi < 10^4$. The lower bound $\xi > 1$ was established in order to provide the validity of the condition $R \gg M^2 \slash (2\xi)$ throughout the \ac{SRA} regime. The upper bound of $\xi < 10^4$ is obtained by resorting to the initial inflationary temperature \cite{reheating}.

As in Eq. \eqref{eq:fourier_mode_preheating}, the decomposition of the scalar field from the \ac{NMC} in Fourier modes yields that each mode is governed by

\begin{equation}
\ddot{\chi}_k + \left( 3H + \dfrac{f^2_R}{f^2} \dot{R} \right) \dot{\chi}_k + \left( \dfrac{k^2}{a^2} + m^2\right) \chi_k = 0.
\end{equation}

\noindent The redefinition $X_k \equiv a^{3/2} \sqrt{f^2} \chi_k$ and the new variable $z$ defined by $2 z = M \left(t - t_0 \right) \pm \pi / 2$ (depending on the sign of $\xi$) allows to transform the previous equation into

\begin{equation}
X_k'' + \left[\left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - 3 \dfrac{H'}{M}-9 \dfrac{H^2}{M^2} + \dfrac{1}{2}\dfrac{f_R^2}{f^2}\left(\dfrac{1}{2}\dfrac{f_R^2}{f^2} R'^2 - 6 \dfrac{HR'}{M} - R'' \right) \right] X_k = 0,
\end{equation}

\noindent where the prime represents a derivative with respect to $z$. Recalling that this action is valid in a $f^2(R) \approx 1$ regime, the above equation can be expanded as,

\begin{equation}
X_k'' + \left[\left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - 3 \dfrac{H'}{M}-9 \dfrac{H^2}{M^2} + + \dfrac{\xi}{M^2} \left( \xi \dfrac{R'^2}{M^2} - 6 \dfrac{H R'}{M} - R'' \right) \right] X_k = 0.
\end{equation}

As discussed before, the fact that after the \ac{SRA} the parameter $z$ answers to the late-time approximation $z \gg 1$ makes the Hubble parameter and curvature go through an oscillatory phase of the type

\begin{equation}
H(z) \simeq \dfrac{M}{3z} \left[1 + \sin (2z) \right],
\qquad\qquad\qquad
R(z) \simeq 3 M H'(z) \simeq \dfrac{2M^2}{z} \cos (2z).
\end{equation}

\noindent This is the path to show that $R''$ term dominates \cite{reheating}, so the equation of $X_k$ can be written as

\begin{equation}
X_k'' + \left[ \left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - \xi \dfrac{R''}{M^2}\right] X_k = 0,
\end{equation}

\noindent which may be written in the form of the Mathieu equation

\begin{equation}
X_k'' + \left[ A_k - 2 q \cos(2z) \right] X_k = 0, \qquad\qquad
A_k = \left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2,
\qquad\qquad q = \dfrac{4\xi}{z}.
\end{equation}

The interesting fact is that with a \ac{NMC} term in the action, the resulting equation is the same as the one obtained in \eqref{eq:mathieu_eq_starobinsky}. The results are, therefore, the same as the ones mentioned in section \ref{sec:reheating}.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Solar System Long Range Impact}
\label{sec:impact_nmc}

Moving forward the parallelism with the pure $f(R)$ case from chapter \ref{cap:fofR}, the \ac{NMC} impact at the Solar System scales is analysed. As in section \ref{sec:solar_sys_impact}, matter is assumed to behave as dust, described by
%
\begin{equation}
T_{\mu\nu} = \rho c^2 u_\mu u_\nu~~~~,~~~~  u_\mu u^\mu =-1,
\end{equation}
%
The trace of the energy-momentum tensor is $T = -\rho c^2$ and the Lagrangian density of matter is treated as $\LL_m = -\rho c^2$.

The function $\rho = \rho(r)$ is again that of a spherically symmetric body with a static radial mass density $\rho = \rho(r)$. This function $\rho(r)$ and its first derivative are assumed to be continuous across the surface of the body,
%
\begin{equation} \label{conditions for fe_march}
\rho(R_S) = 0 \quad \text{and} \quad \dfrac{d\rho}{dr}(R_S) = 0,
\end{equation}
%
\noindent where $R_S$ denotes the radius of the spherical body.

The metric used is once more the perturbed \ac{FLRW} metric, repeated here for convenience:

\begin{equation}
ds^2 = - \left[1 + 2\Psi (r) \right] dt^2 + a(t)^2 \left( \left[1 + 2 \Phi(r) \right] dr^2 + r^2 d\Omega^2 \right),
\label{eq:metric_march}
\end{equation}

\noindent where $\Psi$ and $\Phi$ are perturbing functions such that $\left|\Psi(r)\right| \ll 1$ and $\left|\Phi(r)\right| \ll 1$. The scalar curvature of this spacetime is also expressed as the sum of a time evolving cosmological contribution $R_0(t)$ and a perturbation $R_1(r)$, induced by the local matter distribution,

\begin{equation}
R(r,t) \equiv R_0 (t) + R_1 (r), ~~~~\qquad ~~~~ \left| R_1 (r) \right| \ll R_0 (t).
\label{eq:curvature_march}
\end{equation}

This assumption allows to expand the functions $f^i(R)$ around $R=R_0$ and neglect all the nonlinear terms in $R_1$. This approximation is the same as the one detailed in Eq. \eqref{eq:conditions_linearization_chiba}, with the exception that now both $f^1(R)$ and $f^2(R)$ are subject to it.

\subsection{Solution for the curvature \texorpdfstring{$R_1$}{R1}}

The trace of the field equations \eqref{eq:field_equations_nmc} is
%
\begin{equation} \label{eq:trace_of_field_equations_march}
\left(f^1_R + 2 f^2_R \LL_m \right) R - 2 f^1 =-3 \square
\left(f^1_R + 2 f^2_R \LL_m \right)
+ \left( 1+ f^2 \right) T.
\end{equation}

\noindent Considering the decomposition of the energy-momentum tensor as $T_{\mu\nu} = T^\text{cos}_{\mu\nu} + T^\text{s}_{\mu\nu}$ and of the matter density as $\rho = \rho^\text{cos} (t) + \rho^\text{s} (r)$, the trace equation for the background curvature has the following solution

\begin{equation}
\left(f^1_{R0} + 2 f^2_{R0} \LL^\text{cos}_m \right) R_0 - 2 f_0^1 + 3 \square \left( f^1_{R0} + 2 f^2_{R0} \LL^\text{cos}_m \right) = \left(1 + f^2_0 \right) T^\text{cos}.
\label{eq:solution_trace_eq_background_march}
\end{equation}

Inserting this equation into \eqref{eq:trace_of_field_equations_march} and taking into account that all terms of order $\OO(R_1^2)$ or greater are neglected, yields

\begin{equation}\label{eq:R1_equation_march}
\begin{split}
\left[ -f^1_{R0} +  f^2_{R0}\LL_m + \left( f^1_{RR0} + 2 f^2_{RR0}\LL_m \right) R_0 \right] R_1 + & 3 \square \left[\left( f^1_{RR0} + 2 f^2_{RR0}\LL_m \right) R_1 \right] = \\ 
& \left( 1 +  f^2_0 \right) T^{\rm s} - 2 f^2_{R0}\LL_m^{\rm s}R_0 -
6\square\left( f^2_{R0}\LL_m^{\rm s} \right).
\end{split}
\end{equation}

The expansion of the operator $\square$ and neglecting products of $R_1$ or of its spatial derivatives with $\Psi$ and $\Phi$ and their spatial derivatives, gives the curvature equation the expression

\begin{equation}
\label{eq:U-equation_march}
\nabla^2 U -m^2 U = -\frac{1}{3}\left( 1 +  f^2_0 \right) \rho^{\rm s} +
\frac{2}{3} f^2_{R0}\rho^{\rm s}R_0 + 2 \rho^{\rm s} \square f^2_{R0} +
2 f^2_{R0} \nabla^2 \rho^{\rm s},
\end{equation}

\noindent where the potential $U(r,t)$ is defined as

\begin{equation}\label{eq:potentialdef}
U(r,t) = \left[ f^1_{RR0}(t) + 2 f^2_{RR0}(t)\LL_m(r,t)\right] R_1(r),
\end{equation}
%
and the mass parameter is
%
\begin{equation}
\label{eq:mass-formula_march}
m^2 =  \frac{1}{3}\left[\frac{f^1_{R0} -  f^2_{R0}\LL_m}{f^1_{RR0} + 2 f^2_{RR0}\LL_m}
- R_0 - \frac{3\square\left( f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}\right)
- 6\rho^{\rm s}\square f^2_{RR0}}{f^1_{RR0} + 2 f^2_{RR0}\LL_m} \right],
\end{equation}

\noindent where $f^1_{RR0} + 2 f^2_{RR0}\LL_m \neq 0$ is assumed. Naturally, this expression becomes the one obtained for the pure $f(R)$ theories, Eq. \eqref{eq:trace_equation_chiba_final}, when $f^2(R) = 0$. 

As a first step to work out the solution of the above equation, it is better to consider it outside the star, where $\rho^\text{s} = 0$, so that the mass parameter depends only on time, $m=m(t)$. Equation \eqref{eq:U-equation_march} thus becomes

\begin{equation}
\nabla^2 U = m^2(t) U,
\end{equation}

\noindent and its solution is a Yukawa potential of the type

\begin{equation}
U \sim \dfrac{e^{-mr}}{r},
\end{equation}
%
or, if $m^2 < 0$, an oscillating potential with strength $\sim 1/r$. 

The long range regime condition $mr \ll 1$ means that $U \sim 1 / r$ and so it is possible to neglect the term $m^2 U$ in equation \eqref{eq:U-equation_march}, when computing the total solution of $U(r,t)$. It follows then that equation \eqref{eq:U-equation_march} becomes 

\begin{equation}\label{U-equation-simplified}
\nabla^2 U = \eta(t)\rho^{\rm s}(r) + 2 f^2_{R0} \nabla^2 \rho^{\rm s},
\end{equation}
%
with
%
\begin{equation}\label{etadef}
\eta(t) = -\frac{1}{3}\left( 1 + f^2_0 \right) + \frac{2}{3} f^2_{R0}R_0 + 2 \square f^2_{R0}.
\end{equation}

Computing the solution of $U(r,t)$ outside the body, $r > R_S$, one obtains

\begin{equation}\label{eq:U-equation-simplified-outside}
U(r,t) = -\frac{\eta(t) }{ 4\pi} \frac{M_{\rm S}}{ r},
\end{equation}

\noindent where $M_S$ is the total mass of the spherical body. Through Eq. \eqref{eq:potentialdef}, the curvature $R_1$ is defined as 
%
\begin{equation}\label{eq:R1-solution_march}
R_1(r,t) = \frac{\eta(t) }{ 4\pi \left( 2 f^2_{RR0}\rho^\text{cos}-  f^1_{RR0}\right)} \frac{M_\text{S}}{r},
\end{equation}

\noindent which obviously reduces to Eq. \eqref{eq:curvature_solution_chiba}   when $f^2(R) = 0$. Also, notice that the variation of $R_1$ in time is on a time scale much bigger than the one proper from the Solar system, so that it is plausible to assume $R_1(r,t) \simeq R_1(r)$. The computation of the solution for $r<R_S$ can be found in appendix \ref{ap:curvature}.

\subsection{Solution for \texorpdfstring{$\Psi$}{Psi}}

Using the same linearisation procedure that was used for the curvature, the $tt$ component of the field equations \eqref{eq:field_equations_nmc}  becomes

\begin{equation}
\left( f^1_{R0} + 2 f^2_{R0}\LL_m \right) \left( \nabla^2\Psi + \frac{1}{2}R_1 \right) =
\frac{2}{3} \left(  1 +  f^2_0 +  f^2_{R0}R_0 + 3\square f^2_{R0} \right) \\
\rho^\text{s}.
\label{eq:psi_equation_march}
\end{equation}
%
where Eqs. \eqref{U-equation-simplified} and \eqref{etadef} were also used.

Following section \ref{subsec:long-range}, $\Psi$ is obtained as the sum of two functions, $\Psi = \Psi_0 + \Psi_1$, identified in the equations
%
\begin{equation}\label{eqpsi}
\nabla^2 \Psi_0 = \frac{2}{3} \,\frac{1 +  f^2_0 +  f^2_{R0}R_0 + 3\square f^2_{R0}}
{f^1_{R0} + 2 f^2_{R0}\LL_m} \,\rho^\text{s}, ~~~\qquad\qquad~~
\nabla^2 \Psi_1 = - \frac{1}{2} R_1.
\end{equation}
%
Using the boundary conditions \eqref{conditions for fe} for the matter density, the function $\Psi_0$ outside of the star is obtained through the divergence theorem,
%
\begin{eqnarray}
\nonumber \Psi_0(r,t) &=& -\frac{1}{6\pi}\left( 1 +  f^2_0 +  f^2_{R0}R_0 + 3\square f^2_{R0} \right)
\frac{M^\ast}{ r} + C_0, \\
M^\ast &=& 4\pi \int_0^{R_S} \frac{\rho^{\rm s}(x)}{f^1_{R0} + 2 f^2_{R0}\LL_m(x)}r^2\, dr,
\end{eqnarray}
%
where $C_0$ is an integration constant. The computation of $\Psi_1$ can be found in Ref. \cite{solar}. The most relevant part of the computation is that, under the condition
%
\begin{equation}\label{constraint}
\left\vert\frac{f^1_{R0} + 2 f^2_{R0}\LL_m}{f^1_{RR0} + 2 f^2_{RR0}\LL_m} \right\vert r^2
\ll 1,
\end{equation}
%
considered to be valid inside and outside the spherical body, the function $\Psi_1$ can be written as
%
\begin{eqnarray}
\Psi_1(r,t) &=& \Psi_1^\ast(r,t) + C_1, \\ \nonumber
\left\vert \Psi_1^\ast(r,t) \right\vert &\ll& \left\vert \Psi_0(r,t) - C_0 \right\vert,
\end{eqnarray}
%
where $C_1$ is also an integration constant. Condition Eq. (\ref{constraint}) is satisfied for instance by
functions of the type $f^1(R) \sim R^m$, $f^2(R) \sim R^n$, at least for a suitable range of values of the exponents,
and its meaning will be discussed at the end of this section. \textcolor{red}{[check this sentence]} 
The limit $\lim_{r\to +\infty} \Psi(r,t) = 0$ allows to obtain that $C_0 + C_1 = 0$.
The Newtonian limit also requires that $\Psi(r)$ should be proportional to $M_S \slash r$, leading to the following constraint on the functions $f^1(R)$ and $f^2(R)$:

\begin{equation}\label{Newt-limit}
\left\vert 2 f^2_{R0} \right\vert \rho^\text{s}(r) \ll
\left\vert f^1_{R0} - 2 f^2_{R0}\rho^\text{cos}(t) \right\vert, \qquad r \leq R_S.
\end{equation}

The final solution for $\Psi$ outside of the star is then \textcolor{red}{[I don't get why this is so]},
%
\begin{equation}\label{Psi-solution}
\Psi(r,t) = - \frac{ 1 +  f^2_0 +  f^2_{R0}R_0 + 3\square f^2_{R0} }
{6\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)} \,\frac{M_{S}}{r},
\qquad r \geq R_S.
\end{equation}
%
Once more, this expression reduces to the solution for $\Psi$ from chapter \ref{cap:fofR} if $f^2(R)=0$.

The expression for $\Psi$ can be said to include a gravitational coupling slowly varying in time\footnote{Notice that in this part $G$ is not necessarily Newton's constant, as in the other parts of this text.},
%
\begin{eqnarray}\label{G-constant}
G_\text{eff} &=& \frac{ \omega(t) }
{6\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)}, \\ \nonumber
\omega(t) &=& 1 +  f^2_0 +  f^2_{R0}R_0 +3\square f^2_{R0}.
\end{eqnarray}
%
This expression shows that the timescale $\dot{G}_\text{eff}/G_\text{eff}$ is much bigger than the timescale of the Solar System, thus the approximations $G_\text{eff} \simeq {\rm const.}$ and $\Psi(r,t) \simeq \Psi(r)$ can be made. The available bounds on $\dot{G}_\text{eff}/G_\text{eff}$  \cite{ChibaReview} may help to constrain $f^1(R)$ and $f^2(R)$ through Eq. \eqref{G-constant}.

The solution $R_1$, (\ref{eq:R1-solution_march}), and the effective gravitational constant $G_\text{eff}$, \eqref{G-constant}, are useful to check if $\left\vert R_1 \right\vert \ll R_0$ remains a consistent approximation. Therefore, for $r \geq R_S$,

\begin{equation}
\left\vert\frac{R_1}{R_0}\right\vert \leq \,
\frac{3}{2 R_0}\frac{G_\text{eff}M_{\rm S}}{R_S}
\left\vert\frac{\eta(t)}{\omega(t)}\right\vert \cdot
\left\vert\frac{f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos}}{f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}}\right\vert,
\end{equation}
%
which means that the important assumption $\left\vert R_1 \right\vert \ll R_0$ for the linearisation of the field equations originates another constraint on the functions $f^1(R)$ and $f^2(R)$,
%
\begin{equation}\label{add-constraint}
\left\vert\frac{\eta(t)}{\omega(t)}\right\vert \cdot
\left\vert\frac{f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos}}{f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}}\right\vert
\ll R_0 \left(\frac{R_S}{G_\text{eff}M_{\rm S}}\right).
\end{equation}
%
This is the same as to say that, given the condition,
%
\begin{equation}\label{etaomegaratiocondition}
\left\vert \frac{\eta(t)}{ \omega(t) }\right\vert \lesssim 1 ,
\end{equation}
%
the inequality \eqref{add-constraint} becomes \textcolor{red}{[where do this values come from, the Sun or the Earth?]}
%
\begin{equation}\label{constraint2}
\left\vert\frac{f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos}}{f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}}\right\vert
\ll R_0 \left(\frac{R_S}{G_\text{eff}M_{\rm S}}\right) \approx 4.7 \times 10^5 R_0.
\end{equation}
%
Taking into account the present time value of the Hubble parameter and the fact that $r$ is of the order of the Solar System scales, the approximation $R_0 r^2 \sim H^2 r^2 \ll G_\text{eff}M_{\rm S}/R_S$ can be applied \textcolor{red}{[why?]}, meaning that the condition (\ref{constraint2}) is much stronger than (\ref{constraint}).

Concluding this brief analysis of the solution for $\Psi$, it should be said that when the condition (\ref{constraint2}) is satisfied and the effective gravitational constant $G_\text{eff}$
is identified with Newton's gravitational constant $G$, then Eq. (\ref{add-constraint}) yields $\left\vert R_1 \slash R_0\right\vert \ll 1$. Moreover, the situation when $f^2(R)=0$ once more resumes the conditions from Eqs. (\ref{constraint}) and (\ref{constraint2}) to $\left\vert f^1_{R0}\slash f^1_{RR0} \right\vert r^2 \ll 1$ and $\left\vert f^1_{R0}\slash f^1_{RR0} \right\vert  \ll R_0 R_S/(GM_{\rm s})$ from chapter \ref{cap:fofR}.

\subsection{Solution for \texorpdfstring{$\Phi$}{Phi}}

The solution for $\Phi$ is also obtained through the linearisation of the $rr$ component of the field equations \eqref{eq:field_equations_march}. When $r \geq R_S$ the only matter considered is cosmological background fluid, so that the $rr$ component becomes
%
\begin{equation}\label{Phi-eq-outside}
\left( f^1_{R0} + 2 f^2_{R0}\LL_m^{\rm cos} \right)\left( -\frac{d^2\Psi}{dr^2}
+ \frac{2}{r}\frac{d\Phi}{dr} \right) - \frac{1}{2}f^1_{R0}R_1 + \frac{2}{r}\left(
f^1_{RR0} + 2 f^2_{RR0}\LL_m^{\rm cos} \right) \frac{dR_1}{dr} = 0.
\end{equation}

To simplify this equation it is useful to consider Eq. (\ref{eq:R1-solution_march}) in order to write the following expression

\begin{equation}
\dfrac{R_1}{dR_1\slash dr} = -r,
\end{equation}

\noindent and, taking into account that $\rho^{\rm cos}(t) \ll \rho^{\rm s}(r)$ for $r < R_S$ and that $\left\vert r - R_S \right\vert$ is large enough, to write that the condition (\ref{Newt-limit}) means that

\begin{equation}\label{rhocos-small}
\left\vert 2 f^2_{R0} \right\vert \rho^{\rm cos}(t) \ll \left\vert f^1_{R0} \right\vert.
\end{equation}

\noindent Applying these two expressions to the constraint (\ref{constraint}), gives

\begin{equation}\label{Phi-eq-inside-inequality}
\left\vert \frac{f^1_{R0}R_1 \slash 2}{(2\slash r)
\left( f^1_{RR0} + 2 f^2_{RR0}\LL_m^{\rm cos} \right)\left(dR_1\slash dr\right)} \right\vert \simeq
\frac{1}{4}\left\vert \frac{f^1_{R0} + 2 f^2_{R0}\LL_m^{\rm cos}}
{f^1_{RR0} + 2 f^2_{RR0}\LL_m^{\rm cos}} \right\vert r^2 \ll 1.
\end{equation}

\noindent This allows to neglect the term $f^1_{R0}R_1 \slash 2$ from the $\Phi$ equation (\ref{Phi-eq-outside}), that becomes

\begin{equation}
\frac{d\Phi}{dr} = \frac{r}{2}\, \frac{d^2\Psi}{dr^2} - \left[\frac{f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}}
{f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos}}\right] \, \frac{dR_1}{dr}.
\end{equation}
%
Expanding the derivative terms of $R_1$ and $\Psi$, defined in 
Eqs. (\ref{eq:R1-solution_march}) and (\ref{Psi-solution}), and remembering that $ r \geq R_S$, provides the solution

\begin{equation}
\Phi(r,t) = \frac{1 +  f^2_0 + 4 f^2_{R0}R_0 + 12\square f^2_{R0}}
{12\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)} \,\frac{M_{\rm S}}{r},
\end{equation}

\noindent where $\Phi(r,t) \simeq \Phi(r)$ is once more valid and when $f^2(R)=0$ the solution for $\Phi$ becomes the one from the pure $f(R)$ gravity, \eqref{eq:phi_eq_chiba}.

The PPN parameter $\gamma$ is then
%
\begin{equation}\label{gamma}
\gamma = \frac{1}{2} \, \left[\frac{1 +  f^2_0 + 4 f^2_{R0}R_0 + 12\square f^2_{R0}}
{1 +  f^2_0 +  f^2_{R0}R_0 +3\square f^2_{R0}} \right],
\end{equation}
%
showing that it is completely defined by the background metric $R_0$, whose value is obtained from the cosmological solution of \ac{NMC} gravity, developed in Ref. \cite{nmcexpand}. The case $f^2(R)=0$ obviously yields the value $\gamma = 1\slash 2$ from the computations of chapter \ref{cap:fofR}. 
However, it should be said that this expression for $\gamma$ does not work properly when the functions $f^i (R)$ reduce to their GR expressions, since it implies that the mass parameter $m$, defined in (\ref{eq:mass-formula_march}), is indeed ill-defined (and divergent), so that all the previous assumptions are not satisfied.

Concluding the chapter, all of what was said above means that for a long-range \ac{NMC} model to be compatible with Solar System results, one of these conditions has to be satisfied:
%
\begin{itemize}
\item[{\rm (i)}] The present analysis is not adequate for these tests, because either the condition $|mr| \ll 1$ at Solar System scales shouldn't apply or the nonlinear terms in $R_1$ should be considered in the Taylor expansions from (\ref{eq:conditions_linearization_chiba}) ($i.e.$ the condition $\left\vert R_1 \right\vert \ll R_0$ is not satisfied);
\item[{\rm (ii)}] Or, if both conditions from point (i) are otherwise satisfied, then the validity condition of the Newtonian limit (\ref{Newt-limit}) has to be satisfied, so that the value of $\gamma$ (\ref{gamma}) needs to satisfy the Cassini measurement constraint $\gamma = 1 + (2.1 \pm 2.3) \times 10^{-5}$ \cite{statusgr} \textcolor{red}{]it would be interesting to put here the original cassini paper]}.
\end{itemize}

To advance with condition (ii), the parameter of mass $m^2$ (\ref{eq:mass-formula_march}) needs to be computed with the cosmological solution, $i.e.$ with the values of $R_0(t)$ and $\rho^{\rm cos}(t)$. To do so, the functions $f^i(R)$ should take the form 

\begin{equation}\label{case-study}
f^1(R) = 2\kappa R, \qquad f^2(R) = \left( \frac{R}{R_n} \right)^{-n}, \quad n>0,
\end{equation}
%
where $R_n$ is a constant. These functions are better suited for a cosmological scenario that Ref. \cite{nmcexpand} explains as an expanding one \textcolor{red}{[I hope this is true...]}.

The development of the conditions presented in point (i) in this form of \ac{NMC} gravity is detailed in Ref. \cite{solar}, where the authors make the following conclusions:

\begin{itemize}
\item The Solar System long-range regime $|m| r \ll 1$ leads to $n \gg 10^{-25}$;
\item The validity condition for the Newtonian limit \eqref{Newt-limit} implies that $n \ll 10^{-33}$;
\item The perturbative regime $\left\vert R_1 \right\vert \ll R_0$ leads to an unphysical fine tuning of the density profile $\rho^\text{s}(r)$ inside the spherical body.
\end{itemize}

\noindent The last conclusion related to the lack of validity of the perturbative regime applies to a wide range of astrophysical objects, as long as they are spherical bodies with whom the weak field approximation can be used. Unfortunately this conclusion means that the procedure used in chapter \ref{cap:fofR} \textcolor{red}{[specify the subsection of long-range when the revision of chap2 is made]} does not exclude or even constrain the \ac{NMC} model.

\cleardoublepage


==> 3.Chapter/main3.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dummy Chapter:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% f(R) theories:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Nonminimal Coupling}
\label{cap:nmc}

The remarkable range of applications of $f(R)$ gravity, and in particular the Starobinsky inflationary model, prompted physicists to generalize these theories even further. This generalization is made by a \ac{NMC} between geometry and matter, through the product of the matter Lagrangian density with another function of the curvature, as posited by the action

\begin{equation}\label{eq:action_nmc}
S_\text{NMC}=\int \left[\dfrac{1}{2} f^1(R)+\left[1+f^2(R)\right] \LL_m\right]
\sqrt{-g} d^4x.
\end{equation}

\noindent The field equations, obtained through the variation of the action with respect to the metric, are

\begin{equation} \label{eq:field_equations_nmc}
\left(f^1_R + 2 f^2_R \LL_m \right) R_{\mu \nu} -
\dfrac{1}{2} f^1 g_{\mu \nu} =
\left(1+ f^2 \right) T_{\mu \nu} +\left( \square_{\mu \nu} - g_{\mu \nu} \square \right)
\left( f^1_R + 2 f^2_R \LL_m \right),
\end{equation}

\noindent where $f_R^i \equiv df^i (R) /dR$. If $f^1(R) = 2 \kappa ( R - 2\Lambda)$ and $f^2(R) = 0$, then the action \eqref{eq:action_nmc} collapses to the Einstein-Hilbert action from \eqref{eq:einstein-hilbert_action}.

It should be said that, in opposition to \ac{GR} and pure $f(R)$ gravity, these field equations do not respect the conservation of energy law, $\nabla^\mu T_{\mu\nu} \neq 0$. Indeed, the covariant derivative of the field equations \eqref{eq:field_equations_nmc}, together with the Bianchi identities $\nabla^\mu G_{\mu\nu} = 0$ and the identity

\begin{equation}
(\square \nabla_\nu - \nabla_\nu \square ) f_R^i = R_{\mu\nu} \nabla^\mu f_R^i,
\end{equation}

\noindent yields for the covariant derivative of the energy-momentum tensor,

\begin{equation}
\nabla^\mu T_{\mu\nu} = \dfrac{f_R^2}{1+f^2} \left(g_{\mu\nu} \LL_m - T_{\mu\nu} \right) \nabla^\mu R.
\end{equation}

\noindent Nonetheless, if $f^2(R) = 0$, the pure $f(R)$ case is recovered and the conservation law is fulfilled. This non-conservation of the energy-momentum tensor may yield a violation of the Equivalence principle, for the nonminimal coupling between geometry and matter means that the motion of matter is dependent on the specific form of the Lagrangian density $\LL_m$ and thus matter may not follow the expected geodesic motion.

It should also be mentioned that \ac{NMC} plays an impact on the description of the interior of a central body, leading to a correction to the latter's coupling strength, as is illustrated in Refs. \cite{stelobserv,mimlambda,dynimpac2}.

\section{Scalar-fields equivalence}
\label{sec:scalar-fields}

In section \ref{sec: scalar-fields equiv}, the pure $f(R)$ gravity theories were shown to be equivalent to scalar-tensor theories $-$ in particular, to a \ac{BD} theory of gravity. \ac{NMC} theories of gravity can also be written in a similar way, though with two independent scalar fields. These theories are introduced through the action

\begin{equation}
S = \int \left[ \dfrac{1}{2} f^1 (\phi) + \left[ 1 + f^2 (\phi) \right] \LL_m + \psi (R - \phi) \right] \sqrt{-g} d^4 x,
\label{eq:action_scalar_field_nmc}
\end{equation}

\noindent where $\psi$ acts as a Lagrange multiplier imposing the relation $\phi = R$, with which the action $S$ is reduced to $S_{NMC}$. The variation of this action \eqref{eq:action_scalar_field_nmc} with respect to $\phi$ then yields

\begin{equation}
\psi = \dfrac{1}{2} f^1_R (\phi) + f_R^2 (\phi) \LL_m,
\end{equation}

\noindent which indicates that both scalar-fields are independent if $\LL_m \neq 0$ or $f_R^2 \neq 0$. If $f_R^2=0$, then the action returns to the pure $f(R)$ case.

As in the pure $f(R)$ situation, the action \eqref{eq:action_scalar_field_nmc} can be written in the form of a \ac{BD} theory with $\omega_{BD} = 0$ (check Eq. \eqref{eq:action_brans_dicke}) and the same scalar-fields,

\begin{equation}
S = \int \left[ \psi R - V(\phi,\psi) + \left[ 1 + f^2(\phi) \right] \LL_m \right] \sqrt{-g} d^4x,
\end{equation}

\noindent with the potential

\begin{equation}
V(\phi,\psi) = \phi \psi - \dfrac{1}{2} f^1 (\phi).
\end{equation}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Preheating and Inflation}
\label{sec:preheating}

In section \ref{sec:reheating}, the process of particle production after inflation was explained by means of a preheating mechanism, whose main characteristic was on the parametric resonance of a quantum field $\chi$. The action of this field included a \ac{NMC} term between the curvature and the field itself, of the type $\xi R \chi^2$ $-$ \textit{i.e.} an additional mass term. This linear \ac{NMC} prompts for the more general assumption of the action \eqref{eq:action_nmc} with the functions

\begin{equation}
f^1(R) = 2\kappa \left( R + \dfrac{R^2}{6 M^2} \right), ~~~\qquad\qquad~~~~~~ f^2(R) = 2\xi \dfrac{R}{M^2}.
\end{equation}

\noindent Logically, this specific action has to be able to explain inflation at the standard \ac{SRA}, which means that $f^2(R)$ should interfere only in the preheating situation, and so the \ac{NMC} model only works as part of a perturbative regime with $f^2(R) \sim 0$.

As stated in section \ref{sec:starobinsky}, the mass parameter has the value $M \sim 10^{13}$ GeV$/c^2$, whereas the \ac{NMC} parameter $\xi$ is dimensionless and subject to the range $1 < \xi < 10^4$. The lower bound $\xi > 1$ was established in order to provide the validity of the condition $R \gg M^2 \slash (2\xi)$ throughout the \ac{SRA} regime. The upper bound of $\xi < 10^4$ is obtained by resorting to the initial inflationary temperature \cite{reheating}.

As in Eq. \eqref{eq:fourier_mode_preheating}, the decomposition of the scalar field from the \ac{NMC} in Fourier modes yields that each mode is governed by

\begin{equation}
\ddot{\chi}_k + \left( 3H + \dfrac{f^2_R}{\left(1 + f^2\right)} \dot{R} \right) \dot{\chi}_k + \left( \dfrac{k^2}{a^2} + m^2\right) \chi_k = 0.
\end{equation}

\noindent The redefinition $X_k \equiv a^{3/2} \sqrt{f^2} \chi_k$ and the new variable $z$ defined by $2 z = M \left(t - t_0 \right) \pm \pi / 2$ (depending on the sign of $\xi$) allows to transform the previous equation into

\begin{equation}
X_k'' + \left[\left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - 3 \dfrac{H'}{M}-9 \dfrac{H^2}{M^2} + \dfrac{1}{2}\dfrac{f_R^2}{\left( 1 + f^2\right)}\left(\dfrac{1}{2}\dfrac{f_R^2}{\left( 1 + f^2\right)} R'^2 - 6 \dfrac{HR'}{M} - R'' \right) \right] X_k = 0,
\end{equation}

\noindent where the prime represents a derivative with respect to $z$. Recalling that this action is valid in a $f^2(R) \approx 0$ regime, the above equation can be expanded as,

\begin{equation}
X_k'' + \left[\left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - 3 \dfrac{H'}{M}-9 \dfrac{H^2}{M^2} + + \dfrac{\xi}{M^2} \left( \xi \dfrac{R'^2}{M^2} - 6 \dfrac{H R'}{M} - R'' \right) \right] X_k = 0.
\end{equation}

As discussed before, the fact that after the \ac{SRA} the parameter $z$ answers to the late-time approximation $z \gg 1$ makes the Hubble parameter and curvature go through an oscillatory phase of the type

\begin{equation}
H(z) \simeq \dfrac{M}{3z} \left[1 + \sin (2z) \right],
\qquad\qquad\qquad
R(z) \simeq 3 M H'(z) \simeq \dfrac{2M^2}{z} \cos (2z).
\end{equation}

\noindent This is the path to show that $R''$ term dominates \cite{reheating}, so the equation of $X_k$ can be written as

\begin{equation}
X_k'' + \left[ \left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2 - \xi \dfrac{R''}{M^2}\right] X_k = 0,
\end{equation}

\noindent which may be written in the form of the Mathieu equation

\begin{equation}
X_k'' + \left[ A_k - 2 q \cos(2z) \right] X_k = 0, \qquad\qquad
A_k = \left(\dfrac{2k}{aM}\right)^2 + \left(\dfrac{2m}{M}\right)^2,
\qquad\qquad q = \dfrac{4\xi}{z}.
\end{equation}

The interesting fact is that with a \ac{NMC} term in the action, the resulting equation is the same as the one obtained in \eqref{eq:mathieu_eq_starobinsky}. The results are, therefore, identical to the ones mentioned in section \ref{sec:reheating}.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Solar System Long Range Regime}
\label{sec:impact_nmc}

Moving forward the parallelism with the pure $f(R)$ case from chapter \ref{cap:fofR}, the \ac{NMC} impact at the Solar System scales is analysed. As in section \ref{sec:solar_sys_impact}, matter is assumed to behave as dust, described by Eq. \eqref{eq:conditions_energy_mom_chap2}, so that the trace of the energy-momentum tensor is $T = -\rho c^2$ and the Lagrangian density of matter is treated as $\LL_m = -\rho c^2$.

The function $\rho = \rho(r)$ is again that of a spherically symmetric body with a static radial mass density $\rho = \rho(r)$. This function $\rho(r)$ and its first derivative are assumed to obey Eqs. \eqref{conditions for fe_march}.

The metric used is once more the perturbed \ac{FLRW} metric, repeated here for convenience:

\begin{equation}
ds^2 = - \left[1 + 2\Psi (r) \right] dt^2 + a(t)^2 \left( \left[1 + 2 \Phi(r) \right] dr^2 + r^2 d\Omega^2 \right),
\label{eq:metric_march}
\end{equation}

\noindent where $\Psi$ and $\Phi$ are perturbing functions such that $\left|\Psi(r)\right| \ll 1$ and $\left|\Phi(r)\right| \ll 1$. The scalar curvature of this spacetime is also expressed as the sum of a time evolving cosmological contribution $R_0(t)$ and a perturbation $R_1(r)$, induced by the local matter distribution,

\begin{equation}
R(r,t) \equiv R_0 (t) + R_1 (r), ~~~~\qquad ~~~~ \left| R_1 (r) \right| \ll R_0 (t).
\label{eq:curvature_march}
\end{equation}

This assumption allows to expand the functions $f^i(R)$ around $R=R_0$ and neglect all the nonlinear terms in $R_1$. This approximation is the same as the one detailed in Eq. \eqref{eq:conditions_linearization_chiba}, with the exception that now both $f^1(R)$ and $f^2(R)$ are subject to it.

\subsection{Solution for the curvature \texorpdfstring{$R_1$}{R1}}

The trace of the field equations \eqref{eq:field_equations_nmc} is
%
\begin{equation} \label{eq:trace_of_field_equations_march}
\left(f^1_R + 2 f^2_R \LL_m \right) R - 2 f^1 =-3 \square
\left(f^1_R + 2 f^2_R \LL_m \right)
+ \left( 1+ f^2 \right) T.
\end{equation}

\noindent Considering the decomposition of the energy-momentum tensor as $T_{\mu\nu} = T^\text{cos}_{\mu\nu} + T^\text{s}_{\mu\nu}$ and of the matter density as $\rho = \rho^\text{cos} (t) + \rho^\text{s} (r)$, the trace equation for the background curvature has the following solution

\begin{equation}
\left(f^1_{R0} + 2 f^2_{R0} \LL^\text{cos}_m \right) R_0 - 2 f_0^1 + 3 \square \left( f^1_{R0} + 2 f^2_{R0} \LL^\text{cos}_m \right) = \left(1 + f^2_0 \right) T^\text{cos}.
\label{eq:solution_trace_eq_background_march}
\end{equation}

Inserting this equation into \eqref{eq:trace_of_field_equations_march} and taking into account that all terms of order $\OO(R_1^2)$ or greater are neglected, yields

\begin{equation}\label{eq:R1_equation_march}
\begin{split}
\left[ -f^1_{R0} +  f^2_{R0}\LL_m + \left( f^1_{RR0} + 2 f^2_{RR0}\LL_m \right) R_0 \right] R_1 + & 3 \square \left[\left( f^1_{RR0} + 2 f^2_{RR0}\LL_m \right) R_1 \right] = \\ 
& \left( 1 +  f^2_0 \right) T^{\rm s} - 2 f^2_{R0}\LL_m^{\rm s}R_0 -
6\square\left( f^2_{R0}\LL_m^{\rm s} \right).
\end{split}
\end{equation}

The expansion of the operator $\square$ and neglecting products of $R_1$ or of its spatial derivatives with $\Psi$ and $\Phi$ and their spatial derivatives, gives the curvature equation the expression

\begin{equation}
\label{eq:U-equation_march}
\nabla^2 U -m^2 U = -\frac{1}{3}\left( 1 +  f^2_0 \right) \rho^{\rm s} +
\frac{2}{3} f^2_{R0}\rho^{\rm s}R_0 + 2 \rho^{\rm s} \square f^2_{R0} +
2 f^2_{R0} \nabla^2 \rho^{\rm s},
\end{equation}

\noindent where the potential $U(r,t)$ is defined as

\begin{equation}\label{eq:potentialdef}
U(r,t) = \left[ f^1_{RR0}(t) + 2 f^2_{RR0}(t)\LL_m(r,t)\right] R_1(r),
\end{equation}
%
and the mass parameter is
%
\begin{equation}
\label{eq:mass-formula_march}
m^2 =  \frac{1}{3}\left[\frac{f^1_{R0} -  f^2_{R0}\LL_m}{f^1_{RR0} + 2 f^2_{RR0}\LL_m}
- R_0 - \frac{3\square\left( f^1_{RR0} - 2 f^2_{RR0}\rho^{\rm cos}\right)
- 6\rho^{\rm s}\square f^2_{RR0}}{f^1_{RR0} + 2 f^2_{RR0}\LL_m} \right],
\end{equation}

\noindent where $f^1_{RR0} + 2 f^2_{RR0}\LL_m \neq 0$ is assumed. Naturally, this expression becomes the one obtained for the pure $f(R)$ theories, Eq. \eqref{eq:trace_equation_chiba_final}, when $f^2(R) = 0$. 

As a first step to work out the solution of the above equation, it is better to consider it outside the star, where $\rho^\text{s} = 0$, so that the mass parameter depends only on time, $m=m(t)$. Equation \eqref{eq:U-equation_march} thus becomes

\begin{equation}
\nabla^2 U = m^2(t) U,
\end{equation}

\noindent and its solution is a Yukawa potential of the type

\begin{equation}
U \sim \dfrac{e^{-mr}}{r},
\end{equation}
%
or, if $m^2 < 0$, an oscillating potential with strength $\sim 1/r$. 

The long range regime condition $mr \ll 1$ means that $U \sim 1 / r$ and so it is possible to neglect the term $m^2 U$ in equation \eqref{eq:U-equation_march}, when computing the total solution of $U(r,t)$. It follows then that equation \eqref{eq:U-equation_march} becomes 

\begin{equation}\label{U-equation-simplified}
\nabla^2 U = \eta(t)\rho^{\rm s}(r) + 2 f^2_{R0} \nabla^2 \rho^{\rm s},
\end{equation}
%
with
%
\begin{equation}\label{etadef}
\eta(t) = -\frac{1}{3}\left( 1 + f^2_0 \right) + \frac{2}{3} f^2_{R0}R_0 + 2 \square f^2_{R0}.
\end{equation}

Computing the solution of $U(r,t)$ outside the body, $r > R_S$, one obtains

\begin{equation}\label{eq:U-equation-simplified-outside}
U(r,t) = -\frac{\eta(t) }{ 4\pi} \frac{M_{\rm S}}{ r},
\end{equation}

\noindent where $M_S$ is the total mass of the spherical body. Through Eq. \eqref{eq:potentialdef}, the curvature $R_1$ is defined as 
%
\begin{equation}\label{eq:R1-solution_march}
R_1(r,t) = \frac{\eta(t) }{ 4\pi \left( 2 f^2_{RR0}\rho^\text{cos}-  f^1_{RR0}\right)} \frac{M_\text{S}}{r},
\end{equation}

\noindent which obviously reduces to Eq. \eqref{eq:curvature_solution_chiba}   when $f^2(R) = 0$. Also, notice that the variation of $R_1$ in time is on a time scale much bigger than the one proper from the Solar System, so that it is plausible to assume $R_1(r,t) \simeq R_1(r)$. The $R_1(r)$ solution for $r < R_S$ is not relevant for the following analysis, so it is not presented here (for details, check Ref. \cite{solar}).

\subsection{Solution for \texorpdfstring{$\Psi$}{Psi} and \texorpdfstring{$\Phi$}{Phi}}

The same linearization procedure that was used for the curvature may be used for the $tt$ and $rr$ components of the field equations \eqref{eq:field_equations_nmc}. The computation of $\Psi$ once more goes through a decomposition of the type $\Psi = \Psi_0 + \Psi_1$ and the computation of $\Phi$ is nothing more than a simple integration. The development of these computations is beyond the scope of this section analysis, whose main point is simply to present the results of the long range Solar System effect of the \ac{NMC}. Nonetheless, for more details one should resort to Ref. \cite{solar}.

The final solution for $\Psi$ outside the spherical body is,
%
\begin{equation}\label{Psi-solution}
\Psi(r,t) = - \frac{ 1 +  f^2_0 +  f^2_{R0}R_0 + 3\square f^2_{R0} }
{6\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)} \,\frac{M_{S}}{r},
\qquad r \geq R_S,
\end{equation}
%
which, if $f^2(R)=0$, is reduced to the solution of $\Psi$ from section \ref{subsec:long-range}. This expression can be said to include a gravitational coupling slowly varying in time,
%
\begin{eqnarray}\label{G-constant}
G_\text{eff} &=& \frac{ \omega(t) }
{6\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)}, \\ \nonumber
\omega(t) &=& 1 +  f^2_0 +  f^2_{R0}R_0 +3\square f^2_{R0}.
\end{eqnarray}
%
This expression shows that the timescale $\dot{G}_\text{eff}/G_\text{eff}$ is much bigger than the timescale of the Solar System, and thus the approximations $G_\text{eff} \simeq {\rm const.}$ and $\Psi(r,t) \simeq \Psi(r)$ can be made. The available bounds on $\dot{G}_\text{eff}/G_\text{eff}$  \cite{ChibaReview} may help to constrain $f^1(R)$ and $f^2(R)$ through Eq. \eqref{G-constant}. The Newtonian limit also requires that $\Psi(r)$ should be proportional to $M_S \slash r$, leading to the following constraint on the functions $f^1(R)$ and $f^2(R)$:

\begin{equation}\label{Newt-limit}
\left\vert 2 f^2_{R0} \right\vert \rho^\text{s}(r) \ll
\left\vert f^1_{R0} - 2 f^2_{R0}\rho^\text{cos}(t) \right\vert, \qquad r \leq R_S.
\end{equation}

On the other hand, together with the obtained solutions of $R_1$ and $\Psi$, the $rr$ component of the field equations yields for $\Phi$ the solution

\begin{equation}
\Phi(r,t) = \frac{1 +  f^2_0 + 4 f^2_{R0}R_0 + 12\square f^2_{R0}}
{12\pi \left( f^1_{R0} - 2 f^2_{R0}\rho^{\rm cos} \right)} \,\frac{M_{\rm S}}{r},
\end{equation}

\noindent where $\Phi(r,t) \simeq \Phi(r)$ is once more valid. When $f^2(R)=0$, the solution for $\Phi$ becomes the one from the pure $f(R)$ gravity, \eqref{eq:phi_eq_chiba}.

Having the solutions of both potentials $\Psi$ and $\Phi$, the PPN parameter $\gamma$ is then
%
\begin{equation}\label{gamma}
\gamma = \frac{1}{2} \, \left[\frac{1 +  f^2_0 + 4 f^2_{R0}R_0 + 12\square f^2_{R0}}
{1 +  f^2_0 +  f^2_{R0}R_0 +3\square f^2_{R0}} \right],
\end{equation}
%
showing that it is completely defined by the background metric $R_0$, whose value is obtained from the cosmological solution of \ac{NMC} gravity, developed in Ref. \cite{nmcexpand}. The case $f^2(R)=0$ obviously yields the value $\gamma = 1\slash 2$ from the computations of section \ref{subsec:long-range}. 
However, it should be said that this expression for $\gamma$ does not work properly when the functions $f^i (R)$ reduce to their GR expressions, since it implies that the mass parameter $m$, defined in (\ref{eq:mass-formula_march}), is ill-defined (and divergent), so that many assumptions made to compute $\Psi$ and $\Phi$ are not satisfied \cite{solar}.

Concluding the chapter, all of what was said above means that for a \ac{NMC} model in a long range regime to be compatible with Solar System results, one of these conditions has to be satisfied:
%
\begin{itemize}
\item[{\rm (i)}] The present analysis is not adequate to test the validity of the model, because either the condition $|mr| \ll 1$ at Solar System scales shouldn't apply or the nonlinear terms in $R_1$ should be considered in the Taylor expansions from (\ref{eq:conditions_linearization_chiba}) ($i.e.$ the condition $\left\vert R_1 \right\vert \ll R_0$ is not satisfied);
\item[{\rm (ii)}] Or, if both conditions from point (i) are otherwise satisfied, then the validity condition of the Newtonian limit (\ref{Newt-limit}) has to be satisfied, so that the value of $\gamma$ (\ref{gamma}) needs to satisfy the Cassini measurement constraint $\gamma = 1 + (2.1 \pm 2.3) \times 10^{-5}$ \cite{cassini}.
\end{itemize}

To advance with condition (ii), the parameter of mass $m^2$ (\ref{eq:mass-formula_march}) should be computed with the cosmological solution, \textit{i.e.} with the values of $R_0(t)$ and $\rho^{\rm cos}(t)$. For that, the functions $f^i(R)$ can in general assume power-law forms compatible with the description of the current phase of accelerated expansion of the Universe \cite{nmcexpand,capozziello3}, such as

\begin{equation}
f^1(R) = 2\kappa R, ~~~~~\qquad~~~~~ f^2(R) = \left(\dfrac{R}{R_n}\right)^{-n}, ~~~~ n>0.
\end{equation}

The development of the conditions presented in point (i) in this power-law form of \ac{NMC} gravity is detailed in Ref. \cite{solar}, where the authors make the following conclusions:

\begin{itemize}
\item The Solar System long-range regime $|m| r \ll 1$ leads to $n \gg 10^{-25}$;
\item The validity condition for the Newtonian limit \eqref{Newt-limit} implies that $n \ll 10^{-33}$;
\item The perturbative regime $\left\vert R_1 \right\vert \ll R_0$ leads to an unphysical fine tuning of the density profile $\rho^\text{s}(r)$ inside the spherical body.
\end{itemize}

\noindent The last conclusion is related to the lack of validity of the perturbative regime and it applies to a wide range of astrophysical objects, as long as they are spherical bodies with whom the weak-field approximation can be used. This conclusion means that the procedure used, first applied in section \ref{subsec:long-range}, does not exclude or even constrain the \ac{NMC} model. It is a null-result that nevertheless prompts to inspect more closely the inverse situation of a relevant mass parameter and a negligible cosmological background.

%\cleardoublepage


==> 99.Conclusions/conclusions,_old.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The Introduction:
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Discussion and Outlook}
\label{cap:conclusions}

In this work it has been computed the effect of a \ac{NMC} model, specified by \eqref{f(R) equations}, in a perturbed weak-field Schwarzschild metric, as depicted in Eq. (\ref{psi solution}) and (\ref{phi solution}). In the weak-field limit, this translates into a Yukawa perturbation to the usual Newtonian potential, with characteristic range and coupling strength
%
\begin{equation}
\lambda = \dfrac{1}{m}~~~~,~~~~\alpha = \left( \dfrac{1}{3} - 4\xi \right) = \dfrac{1}{3} \left[ 1 - \left( \dfrac{m}{M} \right)^2 \right]~~.
\end{equation}
%
\noindent This result is quite natural and can be interpreted straightforwardly: a minimally coupled $f(R)$ theory introduces a new massive degree of freedom (as hinted by the equivalence with a scalar-tensor theory \cite{analogy1,analogy2,analogy3}), leading to a Yukawa contribution with characteristic lengthscale $\lambda = 1/m$ and coupling strength $\alpha = 1/3$.

The introduction of a \ac{NMC} has no dynamical effect in the vacuum, as there is no matter to couple the scalar curvature to: as a result, it is not expected any modification in the range of this Yukawa addition. Conversely, a \ac{NMC} has an impact on the description of the interior of the central body leading to a correction to the latter's coupling strength (which has a negative sign since $\LL_m= -\rho$), as mentioned in the beginning of chapter \ref{cap:nmc}.

Using the available experimental constraints, it was found that, for $10^{-22}~{\rm eV} < m < 1~{\rm meV}$ ({\it i.e.} the range $ 10^{-4}~{\rm m} < \lambda < 10^{16}~{\rm m}$), where $|\alpha| \ll 1$, then the \ac{NMC} parameter must be $\xi \sim 1/12$ or, equivalently, both mass scales $m$ and $M$ of the non-trivial functions $f^1(R)$ and $f^2(R)$ must be extremely close.

If this is the case, the latter relation is not interpreted as an undesirable fine-tuning, but instead is suggestive of a common origin for both non-trivial functions $f^1(R)$ and $f^2(R)$, in line with the argument stating that the model \eqref{eq:action_nmc} should arise as a low energy phenomenological approximation to a yet unknown fundamental theory of gravity.

Conversely, for values of $m$ (or $\lambda$) away from the range mentioned above the Yukawa coupling strength, $\alpha$ can be much larger than unity, so that $\xi $ can assume any value and the mass scales $m$ and $M$ can differ considerably.

In particular, the Starobinsky inflationary model, which requires the much heavier mass scale $m \approx 3 \times 10^{13}$ GeV $\sim 10^{-6} M_P$, manifests itself at a lengthscale $\lambda \sim 10^{-29}~{\rm m}$. This implies that the generalized preheating scenario posited in section \ref{sec:reheating} and in Ref. \cite{reheating}, which requires $1<\xi<10^4$, is thus completely allowed by experiment and unconstrained by this work.

By computing the perturbation induced on geodetic precession, it was found that no significant new constraint arises, as this is already included in the existing Yukawa exclusion plot. Furthermore, even considering the much improved precision claimed in a recent study of LAGEOS II --- or, for that matter, any further refinement of $|\alpha| \ll 1$ $-$, no qualitatively new results arise, since this only bridges the gap between $m $ and $M$ ({\it i.e.} narrows the value of $|\xi - 1/12|$).

%\begin{comment}
Finally, a word is due for the so-called chameleon mechanism, first posited in Ref. \cite{chameleon1,chameleon2,chameleon3,chameleon4}, as discussed in Ref. \cite{naff} in relation to $f(R)$ theories. This non-linear effect goes beyond the linear expansion of the modified field equations, and relies on the equivalence between $f(R)$ theories and a scalar-tensor theory with a scalar field $\phi$ proportional to $f_R$, which appears non-minimally coupled to the matter Lagrangian density (in the Einstein frame) \cite{analogy1,analogy2,analogy3,felice}.

As it turns out, the effective potential of this scalar field can be written as $V_{eff}(\phi) = V(\phi) + e^{a\phi}\rho$ (with $a$ an appropriate constant), so that the position of its minimum depends on the density $\rho$, and the mass for the scalar field grows with the density: this is particularly relevant in a cosmological context, where the low background density yields a light, long-ranged field.
%\end{comment}

Given the above, Ref. \cite{naff} speculates that further computations allowing for this non-linear effect could lead to different constraints on the mass scale $m$ of the adopted quadratic form for $f^1(R)$: quite naturally, the inclusion of a direct coupling between curvature ({\it vis-\`a-vis} the scalar field) and matter only heightens this possibility.

Clearly, this prompts for a future study of the relation between this chameleon mechanism and a \ac{NMC} model, in the framework of its equivalence with a multi-scalar-tensor theory as shown in section \ref{sec:scalar-fields}.


\cleardoublepage
